BiomedRAG: A Retrieval Augmented Large Language Model for Biomedicine

Large Language Models (LLMs) have swiftly emerged as vital resources for different applications in the biomedical and healthcare domains; however, these models encounter issues such as generating inaccurate information or hallucinations. Retrieval-augmented generation provided a solution for these models to update knowledge and enhance their performance. In contrast to previous retrieval-augmented LMs, which utilize specialized cross-attention mechanisms to help LLM encode retrieved text, BiomedRAG adopts a simpler approach by directly inputting the retrieved chunk-based documents into the LLM. This straightforward design is easily applicable to existing retrieval and language models, effectively bypassing noise information in retrieved documents, particularly in noise-intensive tasks. Moreover, we demonstrate the potential for utilizing the LLM to supervise the retrieval model in the biomedical domain, enabling it to retrieve the document that assists the LM in improving its predictions. Our experiments reveal that with the tuned scorer,\textsc{ BiomedRAG} attains superior performance across 5 biomedical NLP tasks, encompassing information extraction (triple extraction, relation extraction), text classification, link prediction, and question-answering, leveraging over 9 datasets. For instance, in the triple extraction task, \textsc{BiomedRAG} outperforms other triple extraction systems with micro-F1 scores of 81.42 and 88.83 on GIT and ChemProt corpora, respectively.

==> 8_related_work.tex <==
\section{Related Work}



\subsection{Triple Extraction Methods}
Most previous studies on triple extraction are directed toward employing either the table-filling method~\cite{tang2022unirel,shang2022onerel,liu2023rexuie} or generation methods~\cite{lu2022unified,gao2023easy,fei2022lasuie, lou2023universal,tan2022query}.  For example,  UniRel~\cite{tang2022unirel}  models entity-entity interactions and
entity-relation interactions in one single interaction map, which is predicted by the output probability matrix of auto-encoding language models, such as BERT~\cite{devlin2018bert}.  OneRel~\cite{shang2022onerel} introduces "BIE" (Begin, Inside, End) signs to indicate the position information of a token within entities and utilizes the labeled relationship in BIE to denote the relationship.
% introduces a  Rel-Spec Horns Tagging strategy to predict the entities and their interaction.
UIE~\cite{lu2022unified} explores the ability to universally model various information extraction tasks and adaptively generate the content of the different tasks.
% To address the challenges of UIE neglecting syntax structure information, such as dependency trees, \citet{fei2022lasuie} introduce LasUIE, a unified latent adaptive structure-aware information extraction framework.  
E2H~\cite{gao2023easy} employs a three-stage approach to enhance entity recognition, relation recognition, and triple extraction capabilities.  Compared with all these studies, our focus is on utilizing the retrieval-augmented language model to prompt the model to accurately retrieve chunk information and generate triples.


\subsection{Retrieval-Augmented Language Models (RALMs)}
Many studies~\cite{lewis2020retrieval,guu2020retrieval,gao2023rarr,li2023chain,ram2023context,shi2023replug,li2023understand}, have been proposed to use retrieved information from various knowledge stores to better understand the text or generate the expected output. For example, KIEST~\cite{li2023understand} dynamically injects retrieved entity and attribute knowledge from the knowledge graph when generating the entity or attribute in the task of entity stage changes. RAG~\cite{lewis2020retrieval} uses the maximum inner product search (MIPS) to find the top-K documents which are combined with a query to predict the answers. 
To enhance retrieval capability, RePLUG~\cite{shi2023replug} treats the language model as a black box and enhances retrieval performance by leveraging the language model's output.
% REALM~\cite{guu2020retrieval} employs a gradient-based method to reward the retriever, leading to improved prediction accuracy, while 
% COK~\cite{li2023chain} aims to create a chain of sub-questions and their corresponding queries using a large language model (LLM). Subsequently, they retrieve knowledge relevant to these sub-questions.
Inspired by these studies, we retrieve knowledge from a pre-constructed chunk database and further optimize the retriever using the output of the LLM. As far as we know, we are the first to utilize the RALMs in biomedical triple extraction.


\subsection{Biomedical Triple Extraction Datasets}   %,segura2013semeval,gao2019fewrel,lee2013comagc,van2012eu
% Biomedical triple extraction plays a crucial role in the construction of the medical knowledge graphs and their downstream applications. 

There is some prior research~\cite{khachatrian2019biorelex,gurulingappa2012development,cheng2008polysearch,taboureau2010chemprot} that focuses on biomedical triple extraction dataset construction through expert annotation.  For example,
the BioRelEx~\cite{khachatrian2019biorelex} annotates 2,010 sentences extracted from biomedical literature, specifically addressing binding interactions involving proteins and/or biomolecules.  ADE~\cite{gurulingappa2012development} involves the manual annotation of 4,272 sentences from medical reports, specifically focusing on descriptions of drug-related adverse effects.   
%%%%%%%
DDI~\cite{segura2013semeval} consists of five relation types (mechanism, effect, advice, int, None) extracted from MedLine abstracts.
% PolySearch~\cite{cheng2008polysearch} is an online tool specifically designed for extracting and analyzing two types of relationships (connections, and lack of connection).
Despite their success, these datasets lack sufficient variety in relation types to adequately represent the connections among biomedical entities. Therefore, we introduce GM-CIHT in our work to address this limitation. 
% Additionally, the challenge of data quantity is also noteworthy.
% Our work addresses these concerns by introducing the GM-CIHT  dataset which includes a broader range of relevant biomedical relation types and a larger amount of annotated biomedical sentences.

% In order to investigate domain adaptation capabilities, FewRel 2.0~\cite{gao2019fewrel} created a novel test set sourced from PubMed~\cite{canese2013pubmed}, a comprehensive repository of biomedical sciences data. As a result, they assembled a dataset comprising 25 different relations, each consisting of 100 instances. 

==> 9_preliminaries.tex <==



% \section{Problem Statement}

% In the context of triple extraction, our objective is to extract the triple \textit{(head entity, relation, tail entity)} from the input sentence  $x$. To thoroughly assess the model's extraction capabilities, we introduce a supplementary task, relation extraction, with the objective of predicting the relation type between the provided head entity and tail within the input sentence.

% It's crucial to emphasize that both the training and testing datasets for these tasks consist of the same predefined sets of relations.


% Our objective is to extract the relational triple \textit{(h, r, t)} from a given input sentence  $x$. In this paper, we explore retrieval augmented generation and LLMs to achieve this. To this end, our goal is to first develop a retrieval-augmented LLM framework, which includes constructing a relational key-value memory bank, where the key represents a relation description chunk, and the value corresponds to the respective relation type, i.e., (relation type, relation description chunk). Now, given the input sentence  $x$ .... we use ..... as additional context to generate the target triple ......



==> result_4_17.tex <==


\section{Results}
\label{experiments}
In this section, we present our main results of analysis on BiomedRAG with a focus on several practical facets, including  1) comparative assessments between the \textsc{biomedRAG} framework and other biomedical knowledge extraction models on three datasets, namely GIT, DDI, and ChemProt, 2) comparative assessments between the \textsc{biomedRAG} framework and other biomedical relations extraction framework on GIT-RE, 3) comparative assessments between the \textsc{biomedRAG} framework and other biomedical text classification tasks on ade-corpus-v2 and MTsample. 4) comparative assessments between the \textsc{biomedRAG} framework and other biomedical link prediction tasks on UMLS. 5) model performance under different chunk sizes,  6) Module (tailored chunk scorer, diversity operation) assessment. 7) comparative assessments with RAG models. 



\subsection{Comparative Assessments between Our \textsc{biomedRAG} Framework with Other BioKE  Models }
\label{con:discussuion_triple}

\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc|ccc}
		\toprule 
  
		\multicolumn{1}{c}  {a}&\multicolumn{3}{c}  {DDI}& \multicolumn{3}{c}  {ChemProt} & \multicolumn{3}{c}  {GIT}&\multicolumn{3}{c}  {GIT-RE} \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 &  Precision &  Recall & F1\\
   
	      \midrule
                 GPT-4  &  5.08    &    9.00&  6.50    &  20.79   &37.00   &     26.61& 9.48 & 9.46   &9.47 &48.17 &48.17 & 48.17\\
                 % \hline
                   MedLLaMA 13B~\cite{wu2023pmc} &   76.08   &    76.08  &  76.08      &  69.98  & 69.31 & 69.64 &58.70  & 36.98   & 45.38 &86.42 &86.42 & 86.42 \\
                 MedLLaMA 13B+\textsc{biomedRAG} &   76.90    &76.90    &76.90    & 77.30    & 75.50 & 76.40  & 76.88 & 76.56   &  76.72 & 86.66&86.66 &86.66 \\
                 LLaMA2 13B~\cite{touvron2023llama} &   79.61    &  79.61   &  79.61     &   85.24  &  84.52 &  84.88   &72.14  &  70.75  & 71.44&82.58 & 82.58&82.58 \\
                 LLaMA2 13B + \textsc{biomedRAG} &  \textbf{80.50} &   \textbf{79.10 } &     \textbf{80.00} &   \textbf{89.25}  &  \textbf{88.42} &  \textbf{88.83}  & \textbf{81.78} & \textbf{81.07}   &\textbf{81.42}  &89.03 &89.03 &89.03 \\
           
             \hline
           	\multicolumn{1}{c}  {b}&\multicolumn{3}{c}  {DDI}& \multicolumn{3}{c}  {ChemProt} & \multicolumn{3}{c}  {GIT}&\multicolumn{3}{c}  {GIT-RE} \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 &  Precision &  Recall & F1\\
   
	      \midrule
                 GPT-4  &  5.08    &    9.00&  6.50    &  20.79   &37.00   &     26.61& 9.48 & 9.46   &9.47 &48.17 &48.17 & 48.17\\
                 % \hline
                   MedLLaMA 13B~\cite{wu2023pmc} &   76.08   &    76.08  &  76.08      &  69.98  & 69.31 & 69.64 &58.70  & 36.98   & 45.38 &86.42 &86.42 & 86.42 \\
                 MedLLaMA 13B+\textsc{biomedRAG} &   76.90    &76.90    &76.90    & 77.30    & 75.50 & 76.40  & 76.88 & 76.56   &  76.72 & 86.66&86.66 &86.66 \\
                 LLaMA2 13B~\cite{touvron2023llama} &   79.61    &  79.61   &  79.61     &   85.24  &  84.52 &  84.88   &72.14  &  70.75  & 71.44&82.58 & 82.58&82.58 \\
                 LLaMA2 13B + \textsc{biomedRAG} &  \textbf{80.50} &   \textbf{79.10 } &     \textbf{80.00} &   \textbf{89.25}  &  \textbf{88.42} &  \textbf{88.83}  & \textbf{81.78} & \textbf{81.07}   &\textbf{81.42}  &89.03 &89.03 &89.03 \\
           
           
           
           
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for biomeidcal triple extraction on DDI,  ChemProt and GIT }
\label{con:Model_performance_Chem_DDI_GIT}
\vspace{-1mm}
\end{table*}


\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc}
		\toprule 
  
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {DDI}& \multicolumn{3}{c}  {ChemProt} & \multicolumn{3}{c}  {GIT} \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 \\
   
	      \midrule
		UniRel~\cite{tang2022unirel}  & 25.59  & 21.92& 27.13    &29.00 & 17.45&21.79 &36.36  &  12.50  & 18.60 \\
            % &  QIDN~\cite{tan2022query}& --  &   -- &   -- &    --&  -- & --   & --  &  -- & -- \\
                OneRel~\cite{shang2022onerel} &34.72--  & 81.07--  & 22.09--    &44.95  &45.22  &  44.68 & 47.97 &  52.01  &44.52\\
                UIE (base)~\cite{lu2022unified} & 30.74  &  29.07 & 29.88   &  48.15 &44.79  &46.41  & 34.81 &30.59    &32.56  \\
                UIE (large)~\cite{lu2022unified} &  37.50  & 35.05& 36.24   &    49.74& 46.27    &  47.94 & 33.99 &  29.93  & 31.83  \\
                E2H (base)~\cite{gao2023easy} &  34.23 &   34.25 & 34.24   & 48.92   & 46.51 &47.68    & 31.29 &  26.68  &28.80  \\
                E2H (large)~\cite{gao2023easy}  & 30.24  &  30.16  &    30.20  &  49.86   & 47.78  & 48.80  &31.47  &  26.89  & 29.00  \\
                 GPT-4 (P1)  &  7.35    &  10.00  &   8.47   &  25.00   & 28.00  & 26.42    &  9.51&  9.25  & 9.38\\
                 GPT-4 (P2)  &  5.08    &    9.00&  6.50    &  20.79   &37.00   &     26.61& 9.48 & 9.46   &9.47  \\
                  RA-\textsc{KNN}-n &    77.98&  77.98  &  77.98  &85.55     & 84.61  & 85.08  & 77.92 &77.42    &77.66   \\

                 \hline
                   MedLLaMA 13B~\cite{wu2023pmc} &   76.08   &    76.08  &  76.08      &  69.98  & 69.31 & 69.64 &58.70  & 36.98   & 45.38  \\
                 MedLLaMA 13B+\textsc{biomedRAG} &   76.90    &76.90    &76.90    & 77.30    & 75.50 & 76.40  & 76.88 & 76.56   &  76.72 \\
                 LLaMA2 13B~\cite{touvron2023llama} &   79.61    &  79.61   &  79.61     &   85.24  &  84.52 &  84.88   &72.14  &  70.75  & 71.44\\
                 LLaMA2 13B + \textsc{biomedRAG} &  \textbf{80.50} &   \textbf{79.10 } &     \textbf{80.00} &   \textbf{89.25}  &  \textbf{88.42} &  \textbf{88.83}  & \textbf{81.78} & \textbf{81.07}   &\textbf{81.42}  \\
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for biomeidcal triple extraction on DDI,  ChemProt and GIT }
\label{con:Model_performance_Chem_DDI_GIT}
\vspace{-1mm}
\end{table*}



\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {l|l|ccc|ccc|ccc|ccc}
		\toprule 
  
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Triple}& \multicolumn{3}{c}  {Head Entity}& \multicolumn{3}{c}  {Tail Entity} & \multicolumn{3}{c}  {Relation}  \\
		%\hline
		 &Approach & Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 \\ 

	      \midrule
                
             \multirow{3}*{DDI}&UIE (large)&37.50   & 35.05  & 36.24 &  68.89  &64.40   & 66.57 &  63.37  & 59.24 & 61.23 & 45.63   &  42.66 & 44.10   \\
              &RA-\textsc{KNN}-n  &79.61   & \textbf{79.61}    &79.61     & 95.92 &95.92  &  95.92   &85.05   & 85.05 &  85.05  &  91.57 &  91.57& 91.57   \\
              
               &LLaMA2 13B + \textsc{biomedRAG}& \textbf{80.50} &  79.10 & \textbf{80.00 }& \textbf{97.01}  &\textbf{97.01}  & \textbf{97.01} & \textbf{ 85.59 } &   \textbf{85.59}&\textbf{85.59} &\textbf{92.11}   & \textbf{ 92.10 }&   \textbf{92.12} \\
              \hline
             \multirow{3}*{ChemProt}&E2H (large)&49.86  &  47.78 & 48.80 & 80.45  & 77.09 & 78.73 & 78.23    &74.97   & 76.56&  71.26 & 68.29  &  69.74  \\
              &RA-\textsc{KNN}-n  &  85.55 &84.61 &  85.08    & 98.91  &\textbf{97.81} &\textbf{ 98.36} & 93.08   & 92.05  &92.57 &  91.94 &90.92   &   91.43 \\
               &LLaMA2 13B + \textsc{biomedRAG}& \textbf{89.25} & \textbf{88.42} & \textbf{88.83} & \textbf{98.26}  & 97.35  &97.80   & \textbf{96.71}   &\textbf{95.81}   & \textbf{96.25} &  \textbf{93.01} & \textbf{92.14}  &    \textbf{92.57}\\
                \hline
             \multirow{3}*{GIT}&OneRel &47.97  & 52.01  &  44.52  & 65.26 & 71.54 &60.00   &   68.16   & 75.46  &62.15 & 74.70 & 82.94 & 67.96  \\
                &RA-\textsc{KNN}-n  &  77.92   &77.42 &77.66  & 90.69   &90.10   & 90.39  & 88.74   &  88.17 &  88.45&  83.98& 83.44 &   83.71    \\
            &LLaMA2 13B + \textsc{biomedRAG}&  \textbf{81.78}   & \textbf{81.07 }& \textbf{81.42} & \textbf{92.84} &  \textbf{92.04}  & \textbf{92.44}    &\textbf{91.76}    &\textbf{90.96} & \textbf{91.36}   &   \textbf{87.20} & \textbf{86.45} & \textbf{86.82}   \\
             
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{triple, head entity, tail entity and relation results of various approaches on DDI, ChemProt and GIT}
\label{con:Model_entity_relation_triple}
\vspace{-5mm}
\end{table*}


\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.6\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc}
		\toprule 
  
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {DDI}& \multicolumn{3}{c}  {ChemProt}  \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1\\
                 BiLSTM-CRF + ELMo~\cite{luo2020neural}  &   73.70    &  74.00 &  73.80     &   58.50  & 49.50  &    53.60 \\  
                  Att-BiLSTM-CRF + ELMo~\cite{luo2020neural}   &   75.00   &  75.20 & 75.10    &   59.50  & 51.20  &   55.10 \\  
                 % TPLinker~\cite{wang2020tplinker}   &   71.70  &  74.00 & 72.80   &   61.60  & 59.50  &   60.50  \\  
                  % TRVE~\cite{liu2023joint}   &   81.90  &  78.30&80.10   &  66.80  & 65.70  &  66.30 \\
                  MTMG~\cite{deng2023mtmg}   &  77.20  &  78.20&77.70 &  -- & --  & -- \\
                    JBUIM~\cite{tan2023joint}   &  75.20 & 80.20&77.70 &  69.20& 68.50  & 68.80\\
                 
                 SPBERE~\cite{yang2023spbere}& 78.50  &  79.70&79.20 & 69.70 & 69.80  &69.70 \\
                 
                 \hline
                MedLLaMA 13B~\cite{wu2023pmc} & 76.08      &  76.08   &   76.08    &  69.98  & 69.31 & 69.64   \\
                 MedLLaMA 13B+\textsc{biomedRAG} &   76.90    &76.90    &76.90    & 77.30    & 75.50 & 76.40  \\
                 LLaMA2 13B~\cite{touvron2023llama} &     79.61  & \textbf{79.61}  & 79.61    &   85.24  &  84.52 &  84.88  \\
                 LLaMA2 13B + \textsc{biomedRAG} &  \textbf{80.50} &   79.10  &     \textbf{80.00 }&   \textbf{89.25}  &  \textbf{88.42} &  \textbf{88.83}   \\
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for Biomedical Triple Extraction on DDI and ChemProt. The results are listed from their  source papers.}
\label{con:Model_performance_Chem_DDI_current_baseline}
\vspace{-1mm}
\end{table*}



Table~\ref{con:Model_performance_Chem_DDI_GIT} presents the experiment results of various approaches based on Precision, Recall and F value on the GIT, DDI, and ChemProt. Results are the average over 5 runs.
We have the following observations: On GIT, (1) our \textsc{biomedRAG} significantly outperforms all the strong baselines across all evaluation metrics. (2) we observe that  \textsc{biomedRAG} improve the original    MedLLaMA 13B and LLaMA2 13B  by  31.34\%, 9.98\%  respectively, in terms of Triple-F1. 
(3) We observed that even though our model retrieves only the top-1 document from the diverse chunk database, it still outperforms the KNN-based RA-LLM in retrieving the top-20 documents. 
(4) The performance of lightweight models like UniRel and OneRel significantly lags behind that of the LLaMA2 family, like LLaMA2 7B. 
 %%%%%%%%%%%%
On DDI and ChemProt.
We have the following observations: (1) our \textsc{biomedRAG} still outperforms all baselines across F1 value on these open datasets.  (2) We observe that  \textsc{biomedRAG } improve the original    MedLLaMA 13B and LLaMA2 13B  by 3.92\%, 2.27\%  respectively  on the DDI.  (3) The lower performance observed in Unirel and Onerel can be attributed to the table-filling method struggling to recognize complex biomedical entities or relations. For instance, on DDI, UIE achieves only 61.23\% for tail entity recognition. 

Table~\ref{con:Model_entity_relation_triple} illustrates the entities, relation types, and triple comparisons among the top-2 baseline models and \textsc{biomedRAG}. (1) We observed that \textsc{biomedRAG} achieved state-of-the-art performance in triple F1 value and Relation F1 value. However, on ChemProt, the F1 score for the head entity is lower compared to the RA-KNN-n model. (2) For the lightweight model, such as UIE, it achieves a lower F1 score for relations on the DDI dataset. (3) 
Lightweight models like UIE and OneRel struggle with entity recognition in biomedical sentences, whereas retrieval-based methods could enhance entity recognition performance.


To enhance the model performance, we additionally present the triple extraction results of several state-of-the-art systems sourced from their respective papers. Since the code is not publicly available, we compare their model performance solely on the DDI and ChemProt datasets. Table~\ref{con:Model_performance_Chem_DDI_current_baseline} illustrates these triple extraction results.

\subsection{Comparative Assessments  on the Biomedical Relation Extraction Task}

\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.35\textwidth}{!}{%
	\begin{tabular} {l|ccc}
		\toprule 
		% \multicolumn{1}{c}  {}& \multicolumn{3}{c}  {Relation}  \\
		 Approach & Precision &  Recall & F1 \\ 
		\hline	
        GPT-4 &48.17 & 48.17 & 48.17  \\ %   GPT-4    random 1 sample relation\\
        % &GPT-4 (P2) &  &   &   \\ %   GPT-4    random 1 sample relation\\
        % &Llama 13B~\cite{touvron2023llama}& 86.63  &86.45  &86.54  \\
        RT-1~\cite{li2023far}  &  44.86  &  46.02 & 45.44  \\
        RT-5~\cite{li2023far}  &  44.91  & 46.45 &  45.67 \\
        RT-10~\cite{li2023far}  & 42.80   &43.44   &   43.12\\
        RT-20~\cite{li2023far}  & 44.94   & 45.81  & 45.37  \\
        % \hline
      RA-\textsc{KNN}-n  & 88.38   &88.38  &88.38  \\
        \hline
         LLaMA2 7B&   84.44 & 84.08   &  84.26 \\ 
          LLaMA2 7B + \textsc{biomedRAG}&  86.24  & 86.24       &   86.24  \\
        MedLLaMA 13B& 86.24  &  86.24 & 86.24  \\
        MedLLaMA 13B +  \textsc{biomedRAG}& 86.66 & 86.66    & 86.66 \\   % pertailor-5
         LLaMA2 13B&   82.58  &  82.58    &  82.58  \\
         LLaMA2 13B + \textsc{biomedRAG}&  \textbf{ 89.03}  & \textbf{89.03}   &  \textbf{89.03} \\
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of different approaches in the relation extraction task on the GIT-RE dataset. \textbf{\textsc{biomedRAG}} improves  \textbf{\textsc{LLaMA2 7B }}, \textbf{\textsc{MedLLaMA 13B }}, and \textbf{\textsc{LLaMA2 13B }} by \textbf{1.98\%}, \textbf{0.42\%}, and \textbf{6.45\%}  respectively, in term of F1.}
\label{con:RE performance}
\vspace{-2mm}
\end{table}

The relation extraction task involves predicting the type of relationship between two entities based on a given sentence, head entity, and tail entity. To assess the scalability of our model, in this part, we evaluate the performance of \textsc{biomedRAG} in relation extraction tasks. 
Table~\ref{con:RE performance} presents the experiment results of various approaches. Results 
are the average over 5 runs. We have the following observations: (1) our \textsc{biomedRAG} significantly outperforms all the strong baselines and its variants across all evaluation metrics. (2) We observed that \textsc{biomedRAG } improve the original   \textsc{LLaMA2 7B }, \textsc{MedLLaMA 13B }, and \textsc{LLaMA2 13B }   by \textbf{1.98\%}, \textbf{0.42\%}, and \textbf{6.45\%}  respectively, in term of F1.

\subsection{Comparative Assessments  on the Biomedical Text Classification Task}


\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.6\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ade-corpus-v2}& \multicolumn{3}{c}  {MTsample} \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1 \\
         GPT-4&      &      &       &   &   &   \\
           BERT~\cite{devlin2018bert}&   95.00   & 97.00  &  96.00    &  38.00 &  38.00  &    38.00  \\
            % ClinicalBERT&     &   &      &   &   &     \\
        BioBERT~\cite{lee2020biobert}&  95.00   & 97.00   &   97.00   &  37.00& 37.00 & 37.00\\
            GatorTron~\cite{yang2022gatortron}&   95.00    &  98.00  &  97.00    &  38.00 & 38.00 & 38.00    \\
               % Me LLaMA&   --  &  -- &   --  & 45.10   & 45.10  &  45.10    \\
            
              % RA-KNN-1&  99.60   &  99.60   &   99.60    &    &  cuda:0 &   \\
              % RA-KNN-5&   93.78  & 93.60    &  93.69      &    &   &   \\
              % RA-KNN-10&  93.60   &  93.60    &    93.60     &    &   &   \\
              % RA-KNN-15&  94.20   &    94.20   &   94.20       &    &   &   \\
              % RA-KNN-20&  92.20   &    92.20  &   92.20      &    &   &   \\
              % RA-KNN-25&  90.20   &   90.20    &   90.20       &    &   &   \\
              % RA-KNN-30&  92.20   &  92.20    & 92.20        &    &   &   \\
                \hline
             MedLLaMA 13B~\cite{wu2023pmc} &   94.00 &  94.00 &   94.00  &31.30  &30.80 & 31.05    \\
            MedLLaMA 13B+\textsc{biomedRAG} &  \textbf{99.89}  &  \textbf{99.89} &   \textbf{99.89}  &   32.52  &  32.45 & 32.49  \\
          
             LLaMA2 13B~\cite{touvron2023llama} & 96.20  &   96.20 &   96.20   & 38.00  &38.00  & 38.00     \\
             LLaMA2 13B + \textsc{biomedRAG} & 99.80 &  99.80   &  99.80    &   \textbf{38.50 } & \textbf{38.50}  &\textbf{38.50}   \\
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of different approaches in the biomedical text classification task on the ade-corpus-v2 and MTsample.  }
\label{con:Model_performance_TextClas}
\vspace{-1mm}
\end{table*}



\subsection{Comparative Assessments  on the Biomedical Link Prediction Task}

\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.6\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc}
		\toprule 
              \multicolumn{1}{c}  {}&\multicolumn{3}{c}  {UMLS}& \multicolumn{3}{c}  {AZ} \\
		   Approach & Precision &  Recall & F1& Precision &  Recall & F1 \\ 
		%\hline	
            GPT-4&  6.00   &    6.00  &  6.00     & 33.33  & 33.33  &33.33    \\
            BERT~\cite{devlin2018bert}& 57.00   &  57.00  &  57.00  & 58.15 &58.15  &  58.15\\
            BioBERT~\cite{lee2020biobert}& 58.00   &  58.00  & 58.00  & 59.37&  59.37 &   59.37\\
              GatorTron~\cite{yang2022gatortron}& 59.00   &  59.00  &   59.00  &59.23 &59.23  & 59.23 \\
            %   RA-KNN-1&  59.00   &   59.00    &  59.00  & &  & \\ 
            %   RA-KNN-5&  58.39   &    58.39    &   58.39   & &  &  \\ 
            %   RA-KNN-10&   59.15  &   59.15   &   59.15  & &  & \\ 
            %   RA-KNN-15&   57.63  &     57.63 &   57.63   & &  &\\ 
            %   RA-KNN-20&  55.21   &   55.21    &  55.21  & &  &   \\ 
            %   RA-KNN-25&  55.97  &55.97      &   55.97 & &  & \\ 
            % RA-KNN-30&    55.67 &   55.67    &   55.67   & &  & \\ 
               \hline
             MedLLaMA 13B~\cite{wu2023pmc} & 57.96  &  57.79 &  57.87 &45.56 & 45.56 & 45.56\\
            \textsc{MedLLaMA 13B+biomedRAG}& 58.00 &58.00  &  58.00 &59.16 & 59.16 &59.16 \\
            LLaMA2 13B~\cite{touvron2023llama}& 56.58  &  56.58  & 56.58 &61.94 &61.94  &61.94 \\
             \textsc{LLaMA2 13B+biomedRAG}&\textbf{59.80} &    \textbf{59.80} & \textbf{59.80}  &\textbf{62.22}& \textbf{62.22} & \textbf{62.22}\\   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of different approaches in the biomedical link prediction task on UMLS dataset.}
\label{con:UMLS}
\vspace{-5mm}
\end{table}


Table~\ref{con:UMLS} presents the experiment results of various approaches on the UMLS.  We can see that: (1) We observed that \textsc{biomedRAG } improve the original  \textsc{MedLLaMA 13B }, and \textsc{LLaMA2 13B }   by \textbf{0.13\%},  \textbf{3.22\%}  respectively, in term of F1.  (2) BERT achieves a performance very similar to that of LLaMA2 13B. This suggests that, without special fine-tuning instructions, lightweight models may outperform generation models with large parameters.




% \subsection{Comparative Assessments  on the Biomedical Natural Language Inference Task}
% \begin{table}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.35\textwidth}{!}{%
% 	\begin{tabular} {l|c}
% 		\toprule 
% 		   Approach &  Macro-avg F1 \\ 
% 		%\hline	
%             GPT-4 &  \\
%             PubMedBERT~\cite{gu2021domain}&  73.00 from paper  \\
%              BioLinkBERT~\cite{yasunaga2022linkbert}&     74.00 from paper/43.41   \\
%             BERT~\cite{devlin2018bert}&        \\
%               GatorTron~\cite{yang2022gatortron}& 46.48    \\
%                \hline
%              MedLLaMA 13B~\cite{wu2023pmc} &  60.34    rerun  \\
%             \textsc{MedLLaMA 13B+biomedRAG}&      \\
%             LLaMA2 13B~\cite{touvron2023llama}&  67.26    rerun\\
%              \textsc{LLaMA2 13B+biomedRAG}&    \\   
%            \bottomrule
% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of different approaches in the biomedical natural language inference on BioNLI~\cite{bastan2022bionli} dataset.  the result of  PubMedBERT and  BioLinkBERT are from source paper BioNLI~\cite{bastan2022bionli}}
% \label{con:UMLS}
% \vspace{-5mm}
% \end{table}



\subsection{Comparative Assessments  on the Biomedical Question Answering Task}
\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.3\textwidth}{!}{%
	\begin{tabular} {l|c}
		\toprule 

		   Approach &  accuracy \\ 
            BIOBERT-LARGE&  36.70     \\
            BIOROBERTA&    36.10     \\
            IR-CUSTOM&    36.10    \\
            ROBERTA-LARGE&   35.00   \\
          PubMedBERT &   38.10     \\
           BioLinkBERT &  45.10  \\
            GPT-2 &  33.30      \\
           Galactica-120B& 44.40   \\
           GatorTronGPT-5B  &   40.20      \\
           GatorTronGPT-20B&  45.10  \\
           Me-LLaMA 13B &  49.30 \\
            Me-LLaMA 70B & 62.30 \\
            % \hline
              % Med-PaLM 2~\cite{singhal2023towards}& \textbf{86.50} \\
              %  PMC-LLaMA  13B~\cite{wu2023pmc}& \textbf{56.36} \\
                LLaMA2 13B~\cite{wu2023pmc}(PMC-llama 13b-report)& \textbf{42.73} \\
              %  % \hline
              %    PMC-LLaMA  13B~\cite{wu2023pmc}(me llama-report)& \textbf{45.60} \\
              %         LLaMA2 13B~\cite{wu2023pmc}(me llama-report)& \textbf{46.70} \\
                 GPT-4 (zero-shot)   &  59.15 \\
                   GPT-4+ \textsc{biomedRAG}    &  \textbf{64.61} \\
               % \hline
             % MedLLaMA 13B~\cite{wu2023pmc} &   41.50--  rerunning\\
            
            % \textsc{MedLLaMA 13B+biomedRAG}  &     \\
            % LLaMA2 13B~\cite{touvron2023llama}    &  41.70---rerunning \\
             % \textsc{LLaMA2 13B+biomedRAG}  &    \\   
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of different approaches in the MEDQA (USMLE)~\cite{jin2021disease}.  Med-PaLM 2 results are from \cite{singhal2023towards} }
\label{con:UMLS}
\vspace{-5mm}
\end{table}



% \subsection{Comparative Assessments  on the Biomedical NER Task}
% \begin{table*}[ht]
% 	\centering
%  \renewcommand\arraystretch{1.3}
% \resizebox{0.3\textwidth}{!}{%
% 	\begin{tabular} {l|l | cc }
% 		\toprule 
% 		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}& \multicolumn{2}{c}  {1-shot}\\
% 		&Approach &BC5CDR &NCBI    \\ 
%           \midrule
%          \multirow{12}*{SLMs}&BERT~\cite{devlin2018bert}    &10.58   &  12.33 \\
%          ~&ClinicalBERT~\cite{huang2019clinicalbert} &  19.96  & 8.27  \\ % from allennlp 
%         ~&NNShot~\cite{yang2020simple}   &   32.96 & 11.82   \\
%         ~&BioBERT~\cite{lee2020biobert}   & 36.78   &  27.19 \\
%          ~&StructShot~\cite{yang2020simple}    &16.09& 4.63 \\
%           ~&ContaiNER~\cite{das2022container}    & 37.25 &16.51 \\
%           ~&COPNER~\cite{huang2022copner}  &36.36 &  15.54  \\
%         ~&ProtoBERT~\cite{huang2022copner}   &23.61 &  17.24\\
%         ~&GatorTron~\cite{yang2022large}     & 26.97  & 35.00  \\
%             ~&BINDER~\cite{zhang2023optimizing}  &1.86&  2.95  \\
%          ~&\textsc{W-Procer}~\cite{li2023w}    & 40.26   &38.86 \\
%      ~&MetaNER~\cite{chen2023learning}&     -- &   40.01   \\
%         \midrule
%        \multirow{4}*{LLMs}&Vanilla ICL~\cite{li2023w}  &  43.90 &43.48    \\
%         % ~&GPT-3.5-turbo  & 30.37$\pm$1.26 &  22.60$\pm$1.18   &   39.92$\pm$1.19  & 33.64$\pm$0.55  \\
%         ~&PromptNER~\cite{ashok2023promptner}&   92.84 &   81.29   \\
%           % ~&PromptNER  (just right)&  91.85   &     &      &   \\
%            ~&GPT-NER*~\cite{wang2023gpt}&  91.28  &  90.44     \\
%        ~&GPT-NER*(self-ve)~\cite{wang2023gpt}& 91.28   &  90.79 \\
         
%          ~&RT~\cite{li2023far}&   93.50&   91.56     \\
  
%          % ~&Filter-then-Rerank~\cite{ma2023large}&     -- &  -- &  &    \\
%         \bottomrule            
% 	\end{tabular}
%  }
%   \caption{ The performance comparison of SLMs and LLMs in BC5CDR, and NCBI. self-ve refers to self-verification.
%   }
%   \vspace{+2mm}
% \label{con:Model_performance}
% \end{table*}


\subsection{Model Performance under Different Chunk Sizes}


% \subsection{Analysis}
\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=3in]{chuck_number.pdf}
    }
    \subfigure[]{
	\includegraphics[width=3in]{chuck_number_relation.pdf}
    }
    \quad    %用 \quad 来换行
    \caption{(a): Precision (P), Recall (R), F1 results with different chunk length $m$ settings in the task of biomedical triple extraction task. (b): Precision (P), Recall (R), F1 results with different chunk length $m$ settings in the task of biomedical relation  extraction task. }
    \label{con:chuck_number}
\end{figure}


In our proposed model, there is a parameter that controls the number of chunks: $m\in \{3, 4, 5\}$ when constructing the relational key-value memory, which represents the length of each chunk. This parameter aids in retrieving relevant chuck information, considering that the input sentence often contains noise that can impact generation progress.  In this part, we mainly analyze the impact of the different $m$ in the task of biomedical triple extraction and relation extraction, as shown in Figure~\ref{con:chuck_number}(a) and Figure~\ref{con:chuck_number}(b). 
%%%%%%%%%%%%%
As we can see, in these two tasks, when $m=5$, \textsc{biomedRAG} can construct the more rich relation-based information, and retrieve the more relevant relation chunk to the input sentence.  In addition, the performance of $m=5$ is better than $m=3$ or $m=4$, also indicating that if the granularity of relation chunk is too coarse, it will impact relation recognition and consequently affect model performance.



\subsection{Module (tailored chunk scorer, diversity operation) assessment}


\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.5\textwidth}{!}{%
	\begin{tabular} {l|l|ccc}
		\toprule 
		% \multicolumn{2}{c}  {}& \multicolumn{3}{c}  {triple}  \\
		 &Approach & Precision &  Recall & F1 \\
            \hline
        \multirow{3}*{Triple Extraction}& LLM + \textsc{BIoGAG}&  \textbf{81.78}   & \textbf{81.07 }     & \textbf{81.42} \\
        & LLM+\textsc{BIoGAG }-WTCS&  79.31   &79.14       &79.22     \\ 
        &LLM+\textsc{BIoGAG }-WD&  75.93   &  74.62     & 75.27     \\ 
        \hline
        \multirow{3}*{Relation Extraction}&LLM + \textsc{BIoGAG}&    \textbf{89.03}  &   \textbf{89.03 }  &   \textbf{89.03} \\
        &LLM+\textsc{BIoGAG }-WTCS &86.66   &86.66      &  86.66 \\  
        &LLM+\textsc{BIoGAG }-WD & 85.80  &85.80      & 85.80  \\ 
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{\textsc{BIoGAG} performance about its ablated model. we chose the LLaMA2 13B as
the LLM.}
\label{con:ablated models}
\vspace{-5mm}
\end{table}

The contribution of our model components can also
be learned from ablated models.  In this part, we mainly focus one biomedical triple extraction and relation extraction task. We introduce two
ablated models of \textsc{BIoGAG}, (1) \textsc{BIoGAG}-WTCS
uses a  cosine similarity to choose the most relevant document from diverse chunk database
, without using the Tailored Chunk Scorer.
(2) \textsc{BIoGAG}-WD does not consider the diversity of the chunk database.
In these experiments, we selected LLaMA2 13B + \textsc{BIoGAG} as it demonstrated the highest performance from Table~\ref{con:ablated models}. 
 We find that the performance of \textsc{BIoGAG} degrades as we remove
important model components. Specifically, as shown in Figure.~\ref{con:ablated models} both \textsc{BIoGAG}-WTCS and \textsc{BIoGAG}-WD  perform poorly
when compared to \textsc{BIoGAG}, indicating the importance of training a tailored chunk scorer to adapt the LLM and improve the diversity of chunk database.



\subsection{Comparative Assessments with RAG models}
\label{con:topn-sentence_retrival}
The core of our method design lies in establishing a relational key-value memory at the chunk level and training a tailored chunk scorer to adapt the LLM. To comprehensively assess our model's performance, we conduct a comparative analysis with the prevailing retrieval-based LLM, employing a retriever to obtain the top-$n$ relevant documents related to the input sentence.


More specifically, same as \cite{li2023far, ram2023context}, we employ K-nearest neighbors (KNN) as the retriever to obtain the top-n (sentence, label) pairs from the valid data. For triple extraction tasks, the label comprises the triples.

% , while for relation extraction tasks, the label represents the relation given the head and tail entity.



\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=3in]{triple_extraction_final_c.pdf}
    }
    \subfigure[]{
	\includegraphics[width=3in]{relation_extraction_final_c.pdf}
    }
    \quad    %用 \quad 来换行
    \caption{F1 performance of different models. OneRel stands out as the top SLM, demonstrating the highest F1 performance within the GM-CIHT dataset in our study, surpassing other SLMs.(a): triple extraction (b) relation extraction. BR refers to biomedRAG.}
    \label{con:F1_onerel}
\end{figure}




In the experiment of GM-CIHT, we selected LLaMA2 13B and MedLLaMA 13B as our LLM. Due to input length constraints, we present the performance results for the top-15 in MedLLaMA 13B and top-30 in LLaMA2 13B. As shown in  Figure~\ref{con:F1_onerel}, upon comparing the F1 values between OneRel and MedLLaMA 13B-top-1, we observe that the retrieval-based model proves effective in enhancing triple extraction performance.
%%%%%%%%%%
As depicted in Figure~\ref{con:KNN_retrival}(a) and Figure~\ref{con:KNN_retrival}(b), we observed that the value of $n$ in top-$n$ does not exhibit a direct proportionality with the LLM's performance. Notably, as shown in Figure~\ref{con:F1_onerel}, with the incorporation of \textsc{biomedRAG}, we observed an enhancement in the performance of both MedLLaMA 13B and LLaMA2 13B beyond the best achieved through retrieval alone. For example, the best F1 performance in the triple extraction task for LLaMA2 13B was top-$20$: $77.66$, whereas LLaMA2 13B with \textsc{biomedRAG} achieved 81.42. It is crucial to highlight that while retrieving more sentences can improve performance, it also leads to increased training time.

%%%%%%%%
Consequently, our model also proves effective in reducing training time associated with retrieving additional sentences and addressing challenges related to input length limitations. The experiment results on DDI and Chemprot are shown on Table~\ref{con:DDI_KNN} and ~\ref{con:Chem_KNN}.



\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=3in]{GIT_medllma_KNN.pdf}
    }
    \subfigure[]{
	\includegraphics[width=3in]{GIT_llama213_KNN.pdf}
    }
    \subfigure[]{
	\includegraphics[width=3in]{ ChemProt_llama2.pdf}
    }
     \subfigure[]{
	\includegraphics[width=3in]{ade_corpus_v2_KNN.pdf}
    }

 \subfigure[]{
	\includegraphics[width=3in]{UMLS_llama_2_KNN.pdf}
    }

    
    \quad    %用 \quad 来换行
    \caption{(a): Different F1 performance of  KNN-based retrieval model (by using MedLLaMA 13B) in the task of triple extraction  (TE) and relation extraction (RE). The x-axis refers to the top-n. (b):Different F1 performance of  KNN-based retrieval model (by using LLaMA2 13B) in the task of triple extraction  (TE) and relation extraction (RE). The x-axis refers to the top-n.  }
    \label{con:KNN_retrival}
\end{figure}

%UMLS_llama_2_KNN.pdf

\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.35\textwidth}{!}{%
	\begin{tabular} {l|ccc}
		\toprule 

		\multicolumn{1}{c}  {}& \multicolumn{3}{c}  {Relation}  \\
		 Approach & Precision &  Recall & F1 \\ 
		\hline	
     
        MedLLaMA 13B& 27.74  & 26.45& 27.08 \\
         MedLLaMA 13B-top1& 27.47  & 23.40 & 25.27 \\
        MedLLaMA 13B-top5& 27.73   &23.61  & 25.51 \\
        MedLLaMA 13B-top10& \textbf{32.01}& 20.55 & 25.04 \\
        MedLLaMA 13B-top15&  27.49  &  5.01&8.48  \\
        MedLLaMA 13B +  \textsc{biomedRAG}&31.20 & \textbf{30.10}   &\textbf{31.00} \\   % pertailor-5
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Different F1 performance of KNN-based 
retrieval model (by using MedLLaMA 13B) on DDI.}
\label{con:DDI_KNN}
\vspace{-2mm}
\end{table}



\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.35\textwidth}{!}{%
	\begin{tabular} {l|ccc}
		\toprule 

		\multicolumn{1}{c}  {}& \multicolumn{3}{c}  {Relation}  \\
		 Approach & Precision &  Recall & F1 \\ 
		\hline	
     
        LLamA2 13B& 85.24 &84.52& 84.88 \\
        LLamA2 13B-top1&   85.55   & 84.61& 85.08 \\
        LLamA2 13B-top5& 81.31 &  76.44& 78.80 \\
        LLamA2 13B-top10& 83.94    &82.89   &83.42  \\
         LLamA2 13B-top15& 77.84  & 74.72   & 76.25   \\
        LLamA2 13B-top20& 83.25  & 65.24  &73.15   \\
          LLamA2 13B-top25& 65.79& 33.68  &44.55   \\
            LLamA2 13B-top30&89.25  & 28.27  &  42.94\\
       LLamA2 13B +  \textsc{biomedRAG}&\textbf{89.25} &  \textbf{ 88.42}  & \textbf{88.83}\\   % pertailor-5
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Different F1 performance of KNN-based 
retrieval model (by using LLamA2 13B) on ChemProt}
\label{con:Chem_KNN}
\vspace{-2mm}
\end{table}


==> results_back_4_9.tex <==


\section{Results}
\label{experiments}
In this section, we present our main results of analysis on BiomedRAG with a focus on several practical facets, including  1) data Statistics and comparison with other datasets in the biomedical triple extraction task, 2) comparative assessments between the \textsc{biomedRAG} framework and other biomedical knowledge extraction models on three datasets, namely GIT, DDI, and ChemProt, 3) comparative assessments between the \textsc{biomedRAG} framework and other biomedical relations extraction framework on GIT-RE, 4) comparative assessments between the \textsc{biomedRAG} framework and other biomedical text classification tasks on ade-corpus-v2 and MTsample. 5) comparative assessments between the \textsc{biomedRAG} framework and other biomedical link prediction tasks on UMLS. 6) model performance under different chunk sizes,  7) Module (tailored chunk scorer, diversity operation) assessment. 8) comparative assessments with RAG models. 

\subsection{Data Statistics and Comparison with Other Datasets in the Biomedical Triple Extraction Task}
In Table~\ref{con:Comparison of GM-CIHT}, we show the statistics for GIT as well as the comparable
values for seven   widely-used biomedical triple extraction  datasets,  BioRelEx~\cite{khachatrian2019biorelex}, ADE~\cite{gurulingappa2012development}, CHEMPROT~\cite{taboureau2010chemprot}, DDI~\cite{segura2013semeval}, COMAGC~\cite{lee2013comagc}, EUADR~\cite{van2012eu},
PolySearch~\cite{cheng2008polysearch}. 
GIT  differs from other triple extraction datasets because it includes a broader array of relation types, encompassing 22 distinct types. Additionally, the GIT dataset consists of 4,691 labeled sentences, surpassing the size of all other datasets. This demonstrates
GIT provides a valuable benchmark for biomedical triple extraction. For detailed statistics on each relation type and the respective definitions, please refer to the Appendix~\ref{Statistics for Each Relation Type}.

\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
	\scalebox{0.55}{
	\begin{tabular} {ccccc}
		\hline 
		Dataset& \# Entities &  \#Relation Types&\# sentences \\ 
		\hline	
     BioRelEx~\cite{khachatrian2019biorelex} &9,871  & 1 &  2,010 \\
     ADE~\cite{gurulingappa2012development}&  11,070& 2 &  4,272 \\
      CHEMPROT~\cite{taboureau2010chemprot}&  --&  14 & 3,895   \\
        DDI~\cite{segura2013semeval}&13,107  & 5  &   --  \\
         % FewRel 2.0~\cite{gao2019fewrel}&1294  & 25  & 2500   \\
        COMAGC~\cite{lee2013comagc}& 541 &  15 &  821  \\
           EUADR~\cite{van2012eu}& 339& 4  &  355  \\
            PolySearch~\cite{cheng2008polysearch}& 255 & 2  &  522  \\
    \textbf{GIT (our dataset)} &  \textbf{5,644} & \textbf{22}  &  \textbf{4,691}  \\
  
  % Medical-T& -- &20  & 4352 & 3481/\,440/\,431 \\
		\hline
	\end{tabular}
 }
		\caption{Comparing GIT to the seven commonly used biomedical triple extraction datasets. GIT  contains 3,734 training instances, 465 testing instances, and 492 validation instances. In GIT, the training, testing, and validation datasets each consist of distinct instances, ensuring there are no duplicates or overlaps between them.}
	\label{con:Comparison of GM-CIHT}
\end{table}



\subsection{Comparative Assessments between Our \textsc{biomedRAG} Framework with Other BioKE  Models }
\label{con:discussuion_triple}


\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc|ccc}
		\toprule 
  
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {DDI}& \multicolumn{3}{c}  {ChemProt} & \multicolumn{3}{c}  {GIT} \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1&  Precision &  Recall & F1 \\
   
	      \midrule
		UniRel~\cite{tang2022unirel}  & 25.59  & 21.92& 27.13    &29.00 & 17.45&21.79 &36.36  &  12.50  & 18.60 \\
            % &  QIDN~\cite{tan2022query}& --  &   -- &   -- &    --&  -- & --   & --  &  -- & -- \\
                OneRel~\cite{shang2022onerel} &34.72--  & 81.07--  & 22.09--    &44.95  &45.22  &  44.68 & 47.97 &  52.01  &44.52\\
                UIE (base)~\cite{lu2022unified} & 30.74  &  29.07 & 29.88   &  48.15 &44.79  &46.41  & 34.81 &30.59    &32.56  \\
                UIE (large)~\cite{lu2022unified} &  37.50  & 35.05& 36.24   &    49.74& 46.27    &  47.94 & 33.99 &  29.93  & 31.83  \\
                E2H (base)~\cite{gao2023easy} &  34.23 &   34.25 & 34.24   & 48.92   & 46.51 &47.68    & 31.29 &  26.68  &28.80  \\
                E2H (large)~\cite{gao2023easy}  & 30.24  &  30.16  &    30.20  &  49.86   & 47.78  & 48.80  &31.47  &  26.89  & 29.00  \\
                 % GPT-4 (P1)  &  7.35    &  10.00  &   8.47   &  25.00   & 28.00  & 26.42    &  9.51&  9.25  & 9.38\\
                 % GPT-4 (P2)  &  5.08    &    9.00&  6.50    &  20.79   &37.00   &     26.61& 9.48 & 9.46   &9.47  \\
                  RA-\textsc{KNN}-n &    77.98&  77.98  &  77.98  &85.55     & 84.61  & 85.08  & 77.92 &77.42    &77.66   \\

                 \hline
                   MedLLaMA 13B~\cite{wu2023pmc} &   76.08   &    76.08  &  76.08      &  69.98  & 69.31 & 69.64 &58.70  & 36.98   & 45.38  \\
                 MedLLaMA 13B+\textsc{biomedRAG} &   76.90    &76.90    &76.90    & 77.30    & 75.50 & 76.40  & 76.88 & 76.56   &  76.72 \\
                 LLaMA2 13B~\cite{touvron2023llama} &   79.61    &  79.61   &  79.61     &   85.24  &  84.52 &  84.88   &72.14  &  70.75  & 71.44\\
                 LLaMA2 13B + \textsc{biomedRAG} &  \textbf{80.50} &   \textbf{79.10 } &     \textbf{80.00} &   \textbf{89.25}  &  \textbf{88.42} &  \textbf{88.83}  & \textbf{81.78} & \textbf{81.07}   &\textbf{81.42}  \\
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for biomeidcal triple extraction on DDI,  ChemProt and GIT }
\label{con:Model_performance_Chem_DDI}
\vspace{-1mm}
\end{table*}



\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.8\textwidth}{!}{%
	\begin{tabular} {l|l|ccc|ccc|ccc|ccc}
		\toprule 
  
		\multicolumn{1}{c}  {}&\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {Triple}& \multicolumn{3}{c}  {Head Entity}& \multicolumn{3}{c}  {Tail Entity} & \multicolumn{3}{c}  {Relation}  \\
		%\hline
		 &Approach & Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 &  Precision &  Recall & F1 \\ 

	      \midrule
                \multirow{3}*{GIT}&OneRel &47.97  & 52.01  &  44.52  & 65.26 & 71.54 &60.00   &   68.16   & 75.46  &62.15 & 74.70 & 82.94 & 67.96  \\
                &RA-\textsc{KNN}-n  &  77.92   &77.42 &77.66  & 90.69   &90.10   & 90.39  & 88.74   &  88.17 &  88.45&  83.98& 83.44 &   83.71    \\
            &LLaMA2 13B + \textsc{biomedRAG}&  \textbf{81.78}   & \textbf{81.07 }& \textbf{81.42} & \textbf{92.84} &  \textbf{92.04}  & \textbf{92.44}    &\textbf{91.76}    &\textbf{90.96} & \textbf{91.36}   &   \textbf{87.20} & \textbf{86.45} & \textbf{86.82}   \\
              \hline
             \multirow{3}*{DDI}&UIE (large)&37.50   & 35.05  & 36.24 &  68.89  &64.40   & 66.57 &  63.37  & 59.24 & 61.23 & 45.63   &  42.66 & 44.10   \\
              &RA-\textsc{KNN}-n  &79.61   & 79.61    &79.61     & 95.92 &95.92  &  95.92   &85.05   & 85.05 &  85.05  &  91.57 &  91.57& 91.57   \\
               &LLaMA2 13B + \textsc{biomedRAG}&\textsc{80.50} & \textsc{79.10} & \textsc{80.00} &\textsc{97.01}  &\textsc{97.01}  & \textsc{97.01} &  \textsc{85.59}   &  \textsc{85.59} &\textsc{85.59} &\textsc{92.11}   &  \textsc{92.10} &   \textsc{92.12}  \\
              \hline
             \multirow{3}*{ChemProt}&E2H (large)&49.86  &  47.78 & 48.80 & 80.45  & 77.09 & 78.73 & 78.23    &74.97   & 76.56&  71.26 & 68.29  &  69.74  \\
              &RA-\textsc{KNN}-n  &  85.55 &84.61 &  85.08    & 98.91  &97.81  & 98.36 & 93.08   & 92.05  &92.57 &  91.94 &90.92   &   91.43 \\
               &LLaMA2 13B + \textsc{biomedRAG}&89.25 & 88.42 & 88.83& 98.26  & 97.35  &97.80   & 96.71   &95.81   & 96.25 &  93.01 & 92.14  &    92.57\\
            
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{triple, head entity, tail entity and relation results of various approaches on DDI, ChemProt and GIT}
\label{con:Model main performance}
\vspace{-5mm}
\end{table*}




Table~\ref{con:Model main performance} presents the experiment results of various approaches based on Precision, Recall and F value on the GIT, DDI, and ChemProt. Results are the average over 5 runs.
We have the following observations: On GIT, (1) our \textsc{biomedRAG} significantly outperforms all the strong baselines across all evaluation metrics. (2) we observe that  \textsc{biomedRAG} improve the original    MedLLaMA 13B and LLaMA2 13B  by  31.34\%, 9.98\%  respectively, in terms of Triple-F1. 
% (3) Applying state-of-the-art triple extraction models from the general domain to the biomedical domain exposes their diminished effectiveness, despite their strong performance in the general domain. We hypothesize that the primary cause of the observed results is the failure of these models to discern relationships within complex biomedical sentences, as shown in Table~\ref{con:Model main performance}.
(3) We observed that even though our model retrieves only the top-1 document from the diverse chunk database, it still outperforms the KNN-based RA-LLM in retrieving the top-20 documents. 
% We speculate that the reason for this improvement is that \textsc{biomedRAG} retrieves diverse chunk documents using a tailored chunk scorer, thereby enhancing the model's performance. 
(4) The performance of lightweight models like UniRel and OneRel significantly lags behind that of the LLaMA2 family, like LLaMA2 7B. 
 %%%%%%%%%%%%
On DDI and ChemProt.
% The main reason is that
% the reported results are in the zero-shot setting due to the unavailability of open resources. 
% (6)  UniRel performs significantly worse than OneRel, primarily due to the superiority of the BIE operation in OneRel compared to the Interaction Map in UniRel for entity recognition.
We have the following observations: (1) our \textsc{biomedRAG} still outperforms all baselines across F1 value on these open datasets.  (2) We observe that  \textsc{biomedRAG } improve the original    MedLLaMA 13B and LLaMA2 13B  by 3.92\%, 2.27\%  respectively  on the DDI.  (3) The lower performance observed in Unirel and Onerel can be attributed to the table-filling method struggling to recognize complex biomedical entities or relations. For instance, on DDI, UIE achieves only 61.23\% for tail entity recognition. 





\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.6\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc}
		\toprule 
  
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {DDI}& \multicolumn{3}{c}  {ChemProt}  \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1\\
               
                 BiLSTM-CRF + ELMo~\cite{luo2020neural}  &   73.70    &  74.00 &  73.80     &   58.50  & 49.50  &    53.60 \\  
                  Att-BiLSTM-CRF + ELMo~\cite{luo2020neural}   &   75.00   &  75.20 & 75.10    &   59.50  & 51.20  &   55.10 \\  
                 % TPLinker~\cite{wang2020tplinker}   &   71.70  &  74.00 & 72.80   &   61.60  & 59.50  &   60.50  \\  
                  % TRVE~\cite{liu2023joint}   &   81.90  &  78.30&80.10   &  66.80  & 65.70  &  66.30 \\
                  MTMG~\cite{deng2023mtmg}   &  77.20  &  78.20&77.70 &  -- & --  & -- \\
                    JBUIM~\cite{tan2023joint}   &  75.20 & 80.20&77.70 &  69.20& 68.50  & 68.80\\
                 
                 SPBERE~\cite{yang2023spbere}& 78.50  &  79.70&79.20 & 69.70 & 69.80  &69.70 \\
                 
                 \hline
                MedLLaMA 13B~\cite{wu2023pmc} & 76.08      &  76.08   &   76.08    &  69.98  & 69.31 & 69.64   \\
                 MedLLaMA 13B+\textsc{biomedRAG} &   76.90    &76.90    &76.90    & 77.30    & 75.50 & 76.40  \\
                 LLaMA2 13B~\cite{touvron2023llama} &     79.61  & 79.61  & 79.61    &   85.24  &  84.52 &  84.88  \\
                 LLaMA2 13B + \textsc{biomedRAG} &  80.50 &   79.10  &     80.00 &   \textbf{89.25}  &  \textbf{88.42} &  \textbf{88.83}   \\
           \bottomrule

	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches for biomeidcal triple extraction on DDI and ChemProt.}
\label{con:Model_performance_Chem_DDI}
\vspace{-1mm}
\end{table*}



To assess the generality of the model, we conducted experiments on two widely used biomedical triple extraction datasets: DDI and ChemProt. The model parameters utilized in GM-CIHT are applied to these datasets.
Table~\ref{con:Model_performance_Chem_DDI} displays the experiment results of various approaches based on Precision, Recall, and F-value. We have the following observations: (1) our \textsc{biomedRAG} still outperforms all baselines across F1 value on these open datasets.  (2) We observe that  \textsc{biomedRAG } improve the original    MedLLaMA 13B and LLaMA2 13B  by 3.92\%, 2.27\%  respectively  on the DDI.  The model \textsc{MedLLaMA 13+biomedRAG} achieves a similar performance to the best baseline E2H.  (3) The lower performance observed in Unirel and Onerel can be attributed to the table-filling method struggling to recognize complex biomedical entities or relations. For instance, Unirel achieves only 11\% for tail entity recognition.  While numerous studies in the biomedical domain concentrate on joint entity and relation extraction, there is a scarcity of research reporting triple extraction results specifically for DDI and Chemprot. 


\subsection{Salability on the Relation Extraction Task}
The relation extraction task involves predicting the type of relationship between two entities based on a given sentence, head entity, and tail entity. To assess the scalability of our model and its performance in expert triple extraction tasks, we also evaluate the performance of \textsc{biomedRAG} in relation extraction tasks. The biomedical triple extraction GM-CIHT serves as the source data for the relation extraction task. We convert the GM-CIHT dataset into the relation extraction dataset by using the input context, head entity, and tail entity as model inputs, where the model's output signifies the relationship between the input head entity and tail entity.


% \subsubsection{Dataset}
% The biomedical triple extraction GM-CIHT serves as the source data for the relation extraction task. We convert the GM-CIHT dataset into the relation extraction dataset by using the input context, head entity, and tail entity as model inputs, where the model's output signifies the relationship between the input head entity and tail entity.
% \subsubsection{Baselines}
% % As shown in Figure.~\ref{con:Models in general domain}, we use 8 generally used triple extraction datasets and use the state-of-art model for each dataset as the baselines in our triple extraction task.
% We compare the performance of \textsc{biomedRAG} with several strong baselines based on the LLM, including   \textbf{1) GPT-4}:  In GPT-4, we design prompts to guide the GPT models in predicting relations between the head and tail entities for each input sentence. For more detailed information, please refer to Appendix~\ref{GPT-instruction}.  \textbf{2) RT-n}:  We also employ RT~\cite{li2023far}, a retrieval-augmented and chain-of-thoughts method, to extract the relation between the head and tail entity. $n$ refers the top-$n$ documents. Same as the baselines in our triple extraction task, we consider \textbf{3) LLAMA family} as the baselines: MedLLaMA 13B~\cite{wu2023pmc}, LLaMA2-(7, 13b)~\cite{touvron2023llama}.  
% \textbf{4) RA-LLM}: it is consistent with the RA-LLM in the baseline of the triple extraction task.

\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.35\textwidth}{!}{%
	\begin{tabular} {l|ccc}
		\toprule 
		% \multicolumn{1}{c}  {}& \multicolumn{3}{c}  {Relation}  \\
		 Approach & Precision &  Recall & F1 \\ 
		\hline	
        GPT-4 &48.17 & 48.17 & 48.17  \\ %   GPT-4    random 1 sample relation\\
        % &GPT-4 (P2) &  &   &   \\ %   GPT-4    random 1 sample relation\\
        % &Llama 13B~\cite{touvron2023llama}& 86.63  &86.45  &86.54  \\
        RT-1~\cite{li2023far}  &  44.86  &  46.02 & 45.44  \\
        RT-5~\cite{li2023far}  &  44.91  & 46.45 &  45.67 \\
        RT-10~\cite{li2023far}  & 42.80   &43.44   &   43.12\\
        RT-20~\cite{li2023far}  & 44.94   & 45.81  & 45.37  \\
        % \hline
      RA-\textsc{KNN}-n  & 88.38   &88.38  &88.38  \\
        \hline
         LLaMA2 7B&   84.44 & 84.08   &  84.26 \\ 
          LLaMA2 7B + \textsc{biomedRAG}&  86.24  & 86.24       &   86.24  \\
        MedLLaMA 13B& 86.24  &  86.24 & 86.24  \\
        MedLLaMA 13B +  \textsc{biomedRAG}& 86.66 & 86.66    & 86.66 \\   % pertailor-5
         LLaMA2 13B&   82.58  &  82.58    &  82.58  \\
         LLaMA2 13B + \textsc{biomedRAG}&  \textbf{ 89.03}  & \textbf{89.03}   &  \textbf{89.03} \\
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of different approaches in the relation extraction task. \textbf{\textsc{biomedRAG}} improves  \textbf{\textsc{LLaMA2 7B }}, \textbf{\textsc{MedLLaMA 13B }}, and \textbf{\textsc{LLaMA2 13B }} by \textbf{1.98\%}, \textbf{0.42\%}, and \textbf{6.45\%}  respectively, in term of F1.}
\label{con:RE performance}
\vspace{-2mm}
\end{table}



% \subsubsection{Results and Discussion}
Table~\ref{con:RE performance} presents the experiment results of various approaches. Results 
are the average over 5 runs. We have the following observations: (1) our \textsc{biomedRAG} significantly outperforms all the strong baselines and its variants across all evaluation metrics. (2) We observed that \textsc{biomedRAG } improve the original   \textsc{LLaMA2 7B }, \textsc{MedLLaMA 13B }, and \textsc{LLaMA2 13B }   by \textbf{1.98\%}, \textbf{0.42\%}, and \textbf{6.45\%}  respectively, in term of F1.

% (3) Although MedLLamA 13B is trained on a biomedical dataset, its performance is inferior to that of LLamA2 13B. This underscores the notion that models trained on medical data are not inherently more effective than models trained with diverse data in certain tasks, such as relation extraction.

\subsection{Salability on the text Classification Task}


\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.6\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ade-corpus-v2}& \multicolumn{3}{c}  {MTsample} \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1 \\
           BERT&   95.00   & 97.00  &  96.00    &  38.00 &  38.00  &    38.00  \\
            % ClinicalBERT&     &   &      &   &   &     \\
        BioBERT&  95.00   & 97.00   &   97.00   &  39.00& 39.00 & 39.00\\
            gatortron&   95.00    &  98.00  &  97.00    &  38.00 & 38.00 & 38.00    \\
               % Me LLaMA&   --  &  -- &   --  & 45.10   & 45.10  &  45.10    \\
              \hline
              KNN&  99.60   &  99.60   &   99.60    &    &  cuda:0 &   \\
             MedLLaMA 13B~\cite{wu2023pmc} &   94.00 &  94.00 &   94.00  &35.77   &35.20  & 35.48    \\
            MedLLaMA 13B+\textsc{biomedRAG} &  99.89  &  99.89 &   99.89  &   runing  &   &    \\
          
             LLaMA2 13B~\cite{touvron2023llama} & 96.20  &   96.20 &   96.20   & 39.00  &39.00  & 39.00     \\
             LLaMA2 13B + \textsc{biomedRAG} & 99.80 &  99.80   &  99.80    &     & running  &   \\
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of various approaches. }
\label{con:Model_performance_Chem_DDI}
\vspace{-1mm}
\end{table*}


\subsection{Salability on the link prediction Task}


\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.35\textwidth}{!}{%
	\begin{tabular} {l|ccc}
		\toprule 
		   models & Precision &  Recall & F1 \\ 
		%\hline	
            BERT& 57.00   &  57.00  &  57.00   \\
            BioBERT& 58.00   &  58.00  & 58.00    \\
              gatortron& 59.00   &  59.00  &   59.00  \\
            \hline
            KNN&  59.00   &   59.00    &  59.00   \\ 
             MedLLaMA 13B& 57.96  &  57.79 &  57.87  \\
              \textsc{MedLLaMA 13B+biomedRAG}& 58.00 &58.00  &  58.00  \\
            
                LLaMA 13B~\cite{touvron2023llama}& 56.58  &  56.58  & 56.58  \\
             \textsc{LLaMA 13B+biomedRAG}&59.80 &    59.80 & 59.80  \\   
           \bottomrule
  \hline
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of \textbf{ link prediction}, we choose the MedLLaMA 13B as the LLM as it has a better performance than LLaMA 13B.  2019 n2c2}
\label{con:TC_performance}
\vspace{-5mm}
\end{table}

 

% \subsection{Salability on the Semantic textual similarity Task}


% \begin{table}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.35\textwidth}{!}{%
% 	\begin{tabular} {l|l|ccc}
% 		\toprule 
% 		  Approach & Precision &  Recall & F1 \\ 
% 		%\hline	
%                 ClinicalBERT&   &    & 87.90  \\
%                 GatorTron,90B&   &    & 88.10  \\
%                  GatorTron S,1B&   &    & 85.30   \\
%                  GatorTron S,5B&   &    & 88.80 \\
%                  GatorTron S,10B&   &    & 89.30 \\
%                     GatorTron S,20B&   &    & 89.80 \\
%             LLaMA 13B~\cite{touvron2023llama}&   17.23  &   17.23  &  17.23  \\
%             MedLLaMA 13B&    15.53& 15.53  &   15.53 \\
           
%               \hline
%              \textsc{LLM+biomedRAG}&   &     &   \\   
%            \bottomrule
%   \hline
% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of \textbf{ Semantic textual similarity}, we choose the MedLLaMA 13B as the LLM as it has a better performance than LLaMA 13B.  2019 n2c2}
% \label{con:TC_performance}
% \vspace{-5mm}
% \end{table}


% To further evaluate the salability of our \textsc{biomedRAG}, we also assess the model's performance on the triple classification task, which entails classifying whether a triple belongs to the given sentence or not.


% Table~\ref{con:TC_performance} presents the experiment results of various approaches. Results 
% are the average over 5 runs. We have the following observations: (1) our \textsc{biomedRAG} significantly outperforms all the strong baselines and across all evaluation metrics. (2) We observed that \textsc{biomedRAG } improve the original   \textsc{MedLLaMA 13B },  by \textbf{12.3\%} in term of F1. (3) MedLLamA 13B is trained on a biomedical dataset, its performance is better than LLamA2 13B. (4) 
% GPT-4 still cannot achieve its best performance when tested on the new dataset.

% \begin{table}[ht]
% 	\centering
% 	\renewcommand\arraystretch{1.3}
% \resizebox{0.35\textwidth}{!}{%
% 	\begin{tabular} {l|l|ccc}
% 		\toprule 
% 		  Approach & Precision &  Recall & F1 \\ 
% 		%\hline	
%             LLaMA 13B~\cite{touvron2023llama}&72.25  & 72.25  & 72.25  \\
%             % &PMC-LLaMA 7B~\cite{wu2023pmc}&83.65   &83.65   & 83.65  \\
%             MedLLaMA 13B&  73.69 & 72.90 & 73.29  \\
%             GPT-4&  42.96 & 37.74  &40.18  \\  %   GPT-4    random 1 sample relation
%              RT-1~\cite{li2023far}  &  47.31 & 47.31 & 47.31 \\
%              RT-5~\cite{li2023far} &  52.04 &52.04  &52.04  \\
%              RT-10~\cite{li2023far}  & 48.17  &48.17  &48.17  \\
%              RT-20~\cite{li2023far} & 50.75  & 50.75 & 50.75 \\
%               \hline
%              MedLLaMA KNN-n&  84.08 & 84.08 &84.08 \\
%              \textsc{LLM+biomedRAG}&  \textbf{85.59} &  \textbf{85.59}    & \textbf{85.59} \\   
%            \bottomrule
%   \hline
% 	\end{tabular}
%  }
% \vspace{+2mm}
% \caption{Results of \textbf{triple  classification}, we choose the MedLLaMA 13B as the LLM as it has a better performance than LLaMA 13B.}
% \label{con:TC_performance}
% \vspace{-5mm}
% \end{table}


% It's important to note that while NER performance reports primarily focus on recognizing entities and their labels within a sentence, triple extraction emphasizes identifying both the entities and their connections.



% , the reason is that the F1 performance of our method on entity recognition is 57\%. It remains challenging to recognize some complex biomedical words, such as \textit{halogenated hydrocarbon general anesthetics}.  (3) The lower performance observed in Unirel and Onerel can be attributed to the table-filling method struggling to recognize complex biomedical entities or relations. For instance, Unirel achieves only 11\% for tail entity recognition.

\subsection{Model Performance under Different Chunk Sizes}


% \subsection{Analysis}
\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=3in]{chuck_number.pdf}
    }
    \subfigure[]{
	\includegraphics[width=3in]{chuck_number_relation.pdf}
    }
    \quad    %用 \quad 来换行
    \caption{(a): Precision (P), Recall (R), F1 results with different chunk length $m$ settings in the task of triple extraction (b): Precision (P), Recall (R), F1 results with different chunk length $m$ settings in the task of relation  extraction }
    \label{con:chuck_number}
\end{figure}


In our proposed model, there is a parameter that controls the number of chunks: $m\in \{3, 4, 5\}$ when constructing the relational key-value memory, which represents the length of each chunk. This parameter aids in retrieving relational information, considering that the input sentence often contains noise that can impact relation identification.  We analyze the impact of the different $m$ in the task of triple extraction and relation extraction, as shown in Figure~\ref{con:chuck_number}(a) and Figure~\ref{con:chuck_number}(b). 

% As we can see, in these two tasks, when $m=5$, \textsc{biomedRAG} can construct the more rich relation-based information, and retrieve the more relevant relation chunk to the input sentence.  In addition, the performance of $m=5$ is better than $m=3$ or $m=4$, also indicating that if the granularity of relation chunk is too coarse, it will impact relation recognition and consequently affect model performance.



\subsection{Module (tailored chunk scorer, diversity operation) assessment}


\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.5\textwidth}{!}{%
	\begin{tabular} {l|l|ccc}
		\toprule 
		% \multicolumn{2}{c}  {}& \multicolumn{3}{c}  {triple}  \\
		 &Approach & Precision &  Recall & F1 \\
            \hline
        \multirow{3}*{Triple Extraction}& LLM + \textsc{BIoGAG}&  \textbf{81.78}   & \textbf{81.07 }     & \textbf{81.42} \\
        & LLM+\textsc{BIoGAG }-WTCS&  79.31   &79.14       &79.22     \\ 
        &LLM+\textsc{BIoGAG }-WD&  75.93   &  74.62     & 75.27     \\ 
        \hline
        \multirow{3}*{Relation Extraction}&LLM + \textsc{BIoGAG}&    \textbf{89.03}  &   \textbf{89.03 }  &   \textbf{89.03} \\
        &LLM+\textsc{BIoGAG }-WTCS &86.66   &86.66      &  86.66 \\  
        &LLM+\textsc{BIoGAG }-WD & 85.80  &85.80      & 85.80  \\ 
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{\textsc{BIoGAG} performance about its ablated model. we chose the LLaMA2 13B as
the LLM.}
\label{con:ablated models}
\vspace{-5mm}
\end{table}

The contribution of our model components can also
be learned from ablated models. We introduce two
ablated models of \textsc{BIoGAG}, (1) \textsc{BIoGAG}-WTCS
uses a  cosine similarity to choose the most relevant document from diverse chunk database
, without using the Tailored Chunk Scorer.
(2) \textsc{BIoGAG}-WD does not consider the diversity of the chunk database.
In these experiments, we selected LLaMA2 13B + \textsc{BIoGAG} as it demonstrated the highest performance from Table~\ref{con:Model main performance}. 
 We find that the performance of \textsc{BIoGAG} degrades as we remove
important model components. Specifically, as shown in Figure.~\ref{con:ablated models} both \textsc{BIoGAG}-WTCS and \textsc{BIoGAG}-WD  perform poorly
when compared to \textsc{BIoGAG}, indicating the importance of training a tailored chunk scorer to adapt the LLM and improve the diversity of chunk database.



\subsection{Comparative Assessments with RAG models}
\label{con:topn-sentence_retrival}
The core of our method design lies in establishing a relational key-value memory at the chunk level and training a tailored chunk scorer to adapt the LLM. To comprehensively assess our model's performance, we conduct a comparative analysis with the prevailing retrieval-based LLM, employing a retriever to obtain the top-$n$ relevant documents related to the input sentence.


More specifically, same as \cite{li2023far, ram2023context}, we employ K-nearest neighbors (KNN) as the retriever to obtain the top-n (sentence, label) pairs from the valid data. For triple extraction tasks, the label comprises the triples.

% , while for relation extraction tasks, the label represents the relation given the head and tail entity.



\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=3in]{triple_extraction_final_c.pdf}
    }
    \subfigure[]{
	\includegraphics[width=3in]{relation_extraction_final_c.pdf}
    }
    \quad    %用 \quad 来换行
    \caption{F1 performance of different models. OneRel stands out as the top SLM, demonstrating the highest F1 performance within the GM-CIHT dataset in our study, surpassing other SLMs.(a): triple extraction (b) relation extraction. BR refers to biomedRAG.}
    \label{con:F1_onerel}
\end{figure}




In the experiment of GM-CIHT, we selected LLaMA2 13B and MedLLaMA 13B as our LLM. Due to input length constraints, we present the performance results for the top-15 in MedLLaMA 13B and top-30 in LLaMA2 13B. As shown in  Figure~\ref{con:F1_onerel}, upon comparing the F1 values between OneRel and MedLLaMA 13B-top-1, we observe that the retrieval-based model proves effective in enhancing triple extraction performance.
%%%%%%%%%%
As depicted in Figure~\ref{con:KNN_retrival}(a) and Figure~\ref{con:KNN_retrival}(b), we observed that the value of $n$ in top-$n$ does not exhibit a direct proportionality with the LLM's performance. Notably, as shown in Figure~\ref{con:F1_onerel}, with the incorporation of \textsc{biomedRAG}, we observed an enhancement in the performance of both MedLLaMA 13B and LLaMA2 13B beyond the best achieved through retrieval alone. For example, the best F1 performance in the triple extraction task for LLaMA2 13B was top-$20$: $77.66$, whereas LLaMA2 13B with \textsc{biomedRAG} achieved 81.42. It is crucial to highlight that while retrieving more sentences can improve performance, it also leads to increased training time.

%%%%%%%%
Consequently, our model also proves effective in reducing training time associated with retrieving additional sentences and addressing challenges related to input length limitations. The experiment results on DDI and Chemprot are shown on Table~\ref{con:DDI_KNN} and ~\ref{con:Chem_KNN}.



\begin{figure}[htbp]
    \centering
    \subfigure[]{
        \includegraphics[width=3in]{topn_RE_TE_medLLAMA13b.pdf}
    }
    \subfigure[]{
	\includegraphics[width=3in]{topn_TE_RE_llama2_13b.pdf}
    }
    \quad    %用 \quad 来换行
    \caption{(a): Different F1 performance of  KNN-based retrieval model (by using MedLLaMA 13B) in the task of triple extraction  (TE) and relation extraction (RE). The x-axis refers to the top-n. (b):Different F1 performance of  KNN-based retrieval model (by using LLaMA2 13B) in the task of triple extraction  (TE) and relation extraction (RE). The x-axis refers to the top-n.  }
    \label{con:KNN_retrival}
\end{figure}



\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.35\textwidth}{!}{%
	\begin{tabular} {l|ccc}
		\toprule 

		\multicolumn{1}{c}  {}& \multicolumn{3}{c}  {Relation}  \\
		 Approach & Precision &  Recall & F1 \\ 
		\hline	
     
        MedLLaMA 13B& 27.74  & 26.45& 27.08 \\
         MedLLaMA 13B-top1& 27.47  & 23.40 & 25.27 \\
        MedLLaMA 13B-top5& 27.73   &23.61  & 25.51 \\
        MedLLaMA 13B-top10& \textbf{32.01}& 20.55 & 25.04 \\
        MedLLaMA 13B-top15&  27.49  &  5.01&8.48  \\
        MedLLaMA 13B +  \textsc{biomedRAG}&31.20 & \textbf{30.10}   &\textbf{31.00} \\   % pertailor-5
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Different F1 performance of KNN-based 
retrieval model (by using MedLLaMA 13B) on DDI.}
\label{con:DDI_KNN}
\vspace{-2mm}
\end{table}



\begin{table}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.35\textwidth}{!}{%
	\begin{tabular} {l|ccc}
		\toprule 

		\multicolumn{1}{c}  {}& \multicolumn{3}{c}  {Relation}  \\
		 Approach & Precision &  Recall & F1 \\ 
		\hline	
     
        LLamA2 13B& 85.24 &84.52& 84.88 \\
        LLamA2 13B-top1&   85.55   & 84.61& 85.08 \\
        LLamA2 13B-top5& 81.31 &  76.44& 78.80 \\
        LLamA2 13B-top10& 83.94    &82.89   &83.42  \\
         LLamA2 13B-top15& 77.84  & 74.72   & 76.25   \\
        LLamA2 13B-top20& 83.25  & 65.24  &73.15   \\
          LLamA2 13B-top25& 65.79& 33.68  &44.55   \\
            LLamA2 13B-top30&89.25  & 28.27  &  42.94\\
       LLamA2 13B +  \textsc{biomedRAG}&\textbf{89.25} &  \textbf{ 88.42}  & \textbf{88.83}\\   % pertailor-5
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Different F1 performance of KNN-based 
retrieval model (by using LLamA2 13B) on ChemProt}
\label{con:Chem_KNN}
\vspace{-2mm}
\end{table}



\begin{table*}[ht]
	\centering
	\renewcommand\arraystretch{1.3}
\resizebox{0.6\textwidth}{!}{%
	\begin{tabular} {l|ccc|ccc}
		\toprule 
		\multicolumn{1}{c}  {}&\multicolumn{3}{c}  {ade-corpus-v2}& \multicolumn{3}{c}  {MTsample} \\
		%\hline
		 Approach & Precision &  Recall & F1 &  Precision &  Recall & F1 \\
           BERT~\cite{devlin2018bert}&   95.00   & 97.00  &  96.00    &  38.00 &  38.00  &    38.00  \\
            % ClinicalBERT&     &   &      &   &   &     \\
        BioBERT~\cite{lee2020biobert}&  95.00   & 97.00   &   97.00   &  39.00& 39.00 & 39.00\\
            GatorTron~\cite{yang2022gatortron}&   95.00    &  98.00  &  97.00    &  38.00 & 38.00 & 38.00    \\
               % Me LLaMA&   --  &  -- &   --  & 45.10   & 45.10  &  45.10    \\
            
              RA-KNN-1&  99.60   &  99.60   &   99.60    &    &  cuda:0 &   \\
              RA-KNN-5&   93.78  & 93.60    &  93.69      &    &   &   \\
              RA-KNN-10&  93.60   &  93.60    &    93.60     &    &   &   \\
              RA-KNN-15&  94.20   &    94.20   &   94.20       &    &   &   \\
              RA-KNN-20&  92.20   &    92.20  &   92.20      &    &   &   \\
              RA-KNN-25&  90.20   &   90.20    &   90.20       &    &   &   \\
              RA-KNN-30&  92.20   &  92.20    & 92.20        &    &   &   \\
                \hline
             MedLLaMA 13B~\cite{wu2023pmc} &   94.00 &  94.00 &   94.00  &35.77   &35.20  & 35.48    \\
            MedLLaMA 13B+\textsc{biomedRAG} &  \textbf{99.89}  &  \textbf{99.89} &   \textbf{99.89}  &   runing  &   &    \\
          
             LLaMA2 13B~\cite{touvron2023llama} & 96.20  &   96.20 &   96.20   & 39.00  &39.00  & 39.00     \\
             LLaMA2 13B + \textsc{biomedRAG} & 99.80 &  99.80   &  99.80    &   38.50  & 38.50  &38.50   \\
           \bottomrule
	\end{tabular}
 }
\vspace{+2mm}
\caption{Results of different approaches in the biomedical text classification task on the ade-corpus-v2 and MTsample.  }
\label{con:Model_performance_TextClas}
\vspace{-1mm}
\end{table*}

